Hardware-friendly IR-HARQ for Polar SCL Decoders

To extend the applications of polar codes within next-generation wireless communication systems, it is essential to incorporate support for Incremental Redundancy (IR) Hybrid Automatic Repeat Request (HARQ) schemes. The baseline IR-HARQ scheme's reliance on set-based operations leads to irregular memory access patterns, posing significant challenges for efficient hardware implementation. Furthermore, the introduction of new bit types increases the number of fast nodes that are decoded without traversing the sub-tree, resulting in a substantial area overhead when implemented in hardware. To address these issues and improve hardware compatibility, we propose transforming the set-based operations within the polar IR-HARQ scheme into binary vector operations. Additionally, we introduce a new fast node integration approach that avoids increasing the number of fast nodes, thereby minimizing the associated area overhead. Our proposed scheme results in a memory overhead of 25-27% compared to successive cancellation list (SCL) decoding without IR-HARQ support.

==> plots/mine/Q2048.tex <==
% |-------|-------------- |-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |  FMEMA   |  BMEMA   |   MBMEM  |   MFMEM  |   FLOPS  |   BOPS   |
% |-------|---------------|-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
   -1.50 |          -1.50 |            101 |    51200 |      101 | 2.48e-01 | 1.00e+00 | 4.41e+04 | 0.00e+00 |   160563 |        0 | 2.46e+03 | 3.11e+03 | 
   -1.00 |          -1.00 |            101 |    51269 |      101 | 2.48e-01 | 1.00e+00 | 4.41e+04 | 0.00e+00 |   160563 |        0 | 2.46e+03 | 3.11e+03 | 
   -0.50 |          -0.50 |            101 |    51169 |      101 | 2.47e-01 | 1.00e+00 | 4.41e+04 | 0.00e+00 |   160563 |        0 | 2.46e+03 | 3.11e+03 | 
    0.00 |           0.00 |            101 |    50181 |      101 | 2.43e-01 | 1.00e+00 | 4.41e+04 | 0.00e+00 |   160547 |        0 | 2.46e+03 | 3.11e+03 | 
    0.50 |           0.50 |            107 |    43785 |      101 | 2.00e-01 | 9.44e-01 | 8.05e+04 | 0.00e+00 |   217512 |        0 | 4.52e+03 | 4.16e+03 | 
    1.00 |           1.00 |            260 |    36357 |      101 | 6.83e-02 | 3.88e-01 | 2.48e+05 | 0.00e+00 |   964560 |        0 | 1.39e+04 | 8.73e+03 | 
    1.50 |           1.50 |           1806 |    29797 |      101 | 8.06e-03 | 5.59e-02 | 1.99e+05 | 0.00e+00 |  4796339 |        0 | 1.11e+04 | 6.31e+03 | 
    2.00 |           2.00 |          56788 |    23258 |      101 | 2.00e-04 | 1.78e-03 | 1.76e+05 | 0.00e+00 | 130193743 |        0 | 9.82e+03 | 5.44e+03 | 

==> plots/mine/Q3072.tex <==
% |-------|-------------- |-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |  FMEMA   |  BMEMA   |   MBMEM  |   MFMEM  |   FLOPS  |   BOPS   |
% |-------|---------------|-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
   -4.24 |          -6.00 |            101 |    51709 |      101 | 2.50e-01 | 1.00e+00 | 1.19e+05 | 0.00e+00 |   382534 |        0 | 6.27e+03 | 7.35e+03 | 
   -3.74 |          -5.50 |            101 |    51549 |      101 | 2.49e-01 | 1.00e+00 | 1.19e+05 | 0.00e+00 |   382486 |        0 | 6.27e+03 | 7.35e+03 | 
   -3.24 |          -5.00 |            101 |    51452 |      101 | 2.49e-01 | 1.00e+00 | 1.19e+05 | 0.00e+00 |   382470 |        0 | 6.27e+03 | 7.35e+03 | 
   -2.74 |          -4.50 |            101 |    51514 |      101 | 2.49e-01 | 1.00e+00 | 1.18e+05 | 0.00e+00 |   382022 |        0 | 6.23e+03 | 7.32e+03 | 
   -2.24 |          -4.00 |            101 |    51645 |      101 | 2.50e-01 | 1.00e+00 | 1.18e+05 | 0.00e+00 |   381814 |        0 | 6.21e+03 | 7.31e+03 | 
   -1.74 |          -3.50 |            101 |    51866 |      101 | 2.51e-01 | 1.00e+00 | 1.17e+05 | 0.00e+00 |   381510 |        0 | 6.18e+03 | 7.28e+03 | 
   -1.24 |          -3.00 |            101 |    51342 |      101 | 2.48e-01 | 1.00e+00 | 1.17e+05 | 0.00e+00 |   381422 |        0 | 6.17e+03 | 7.28e+03 | 
   -0.74 |          -2.50 |            101 |    51083 |      101 | 2.47e-01 | 1.00e+00 | 1.17e+05 | 0.00e+00 |   381394 |        0 | 6.17e+03 | 7.28e+03 | 
   -0.24 |          -2.00 |            104 |    47428 |      101 | 2.23e-01 | 9.71e-01 | 1.13e+05 | 0.00e+00 |   381234 |        0 | 5.99e+03 | 7.06e+03 | 
    0.26 |          -1.50 |            166 |    39832 |      101 | 1.17e-01 | 6.08e-01 | 2.84e+05 | 0.00e+00 |   932832 |        0 | 1.50e+04 | 1.45e+04 | 
    0.76 |          -1.00 |            814 |    36691 |      101 | 2.20e-02 | 1.24e-01 | 5.35e+05 | 0.00e+00 |  7000370 |        0 | 2.83e+04 | 2.56e+04 | 
    1.26 |          -0.50 |          16811 |    29586 |      101 | 8.59e-04 | 6.01e-03 | 3.87e+05 | 0.00e+00 | 101879658 |        0 | 2.05e+04 | 1.84e+04 | 
    1.76 |           0.00 |         146804 |     9319 |       28 | 3.10e-05 | 1.91e-04 | 5.57e+05 | 0.00e+00 | 1416487266 |        0 | 2.90e+04 | 2.55e+04 | 

==> plots/mine/Q4092.tex <==
% |-------|-------------- |-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |  FMEMA   |  BMEMA   |   MBMEM  |   MFMEM  |   FLOPS  |   BOPS   |
% |-------|---------------|-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
   -2.99 |          -6.00 |            101 |    51611 |      101 | 2.50e-01 | 1.00e+00 | 2.04e+05 | 0.00e+00 |   512437 |        0 | 1.05e+04 | 1.18e+04 | 
   -2.49 |          -5.50 |            101 |    51640 |      101 | 2.50e-01 | 1.00e+00 | 2.04e+05 | 0.00e+00 |   512237 |        0 | 1.05e+04 | 1.18e+04 | 
   -1.99 |          -5.00 |            101 |    51549 |      101 | 2.49e-01 | 1.00e+00 | 2.04e+05 | 0.00e+00 |   512213 |        0 | 1.05e+04 | 1.18e+04 | 
   -1.49 |          -4.50 |            101 |    51533 |      101 | 2.49e-01 | 1.00e+00 | 2.03e+05 | 0.00e+00 |   511733 |        0 | 1.05e+04 | 1.17e+04 | 
   -0.99 |          -4.00 |            101 |    50142 |      101 | 2.42e-01 | 1.00e+00 | 2.02e+05 | 0.00e+00 |   511453 |        0 | 1.05e+04 | 1.17e+04 | 
   -0.49 |          -3.50 |            104 |    46073 |      101 | 2.16e-01 | 9.71e-01 | 1.96e+05 | 0.00e+00 |   511141 |        0 | 1.01e+04 | 1.14e+04 | 
    0.01 |          -3.00 |            177 |    36289 |      101 | 1.00e-01 | 5.71e-01 | 4.60e+05 | 0.00e+00 |  1451860 |        0 | 2.38e+04 | 2.37e+04 | 
    0.51 |          -2.50 |            994 |    28352 |      101 | 1.39e-02 | 1.02e-01 | 8.59e+05 | 0.00e+00 | 13367666 |        0 | 4.45e+04 | 4.27e+04 | 
    1.01 |          -2.00 |          33870 |    19010 |      101 | 2.74e-04 | 2.98e-03 | 7.09e+05 | 0.00e+00 | 419630680 |        0 | 3.60e+04 | 3.42e+04 | 
    1.51 |          -1.50 |          89699 |     3211 |       15 | 1.75e-05 | 1.67e-04 | 2.09e+06 | 0.00e+00 | 3279484208 |        0 | 1.07e+05 | 1.00e+0

==> plots/mine/Q5120.tex <==
% |-------|-------------- |-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |  FMEMA   |  BMEMA   |   MBMEM  |   MFMEM  |   FLOPS  |   BOPS   |
% |-------|---------------|-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
   -2.02 |          -6.00 |            101 |    51296 |      101 | 2.48e-01 | 1.00e+00 | 3.42e+05 | 0.00e+00 |   971140 |        0 | 1.71e+04 | 1.96e+04 | 
   -1.52 |          -5.50 |            101 |    51210 |      101 | 2.48e-01 | 1.00e+00 | 3.42e+05 | 0.00e+00 |   970940 |        0 | 1.71e+04 | 1.96e+04 | 
   -1.02 |          -5.00 |            101 |    49513 |      101 | 2.39e-01 | 1.00e+00 | 3.42e+05 | 0.00e+00 |   970892 |        0 | 1.71e+04 | 1.96e+04 | 
   -0.52 |          -4.50 |            103 |    47058 |      101 | 2.23e-01 | 9.81e-01 | 3.34e+05 | 0.00e+00 |   970406 |        0 | 1.67e+04 | 1.92e+04 | 
   -0.02 |          -4.00 |            198 |    40413 |      101 | 9.97e-02 | 5.10e-01 | 1.22e+06 | 0.00e+00 |  4536738 |        0 | 6.08e+04 | 6.45e+04 | 
    0.48 |          -3.50 |           1484 |    39070 |      101 | 1.29e-02 | 6.81e-02 | 6.01e+05 | 0.00e+00 | 15822740 |        0 | 3.01e+04 | 3.16e+04 | 
  0.98 |          -3.00 |          20924 |    39452 |      101 | 9.21e-04 | 4.83e-03 | 1.32e+06 | 0.00e+00 | 546993734 |        0 | 6.51e+04 | 6.32e+04 | 
  1.48 |          -2.50 |         208992 |    14330 |       39 | 3.35e-05 | 1.87e-04 | 1.09e+06 | 0.00e+00 | 4076845780 |  


==> plots/mine/Q6144.tex <==
% |-------|-------------- |-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |  FMEMA   |  BMEMA   |   MBMEM  |   MFMEM  |   FLOPS  |   BOPS   |
% |-------|---------------|-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
   -1.23 |          -6.00 |            101 |    49671 |      101 | 2.40e-01 | 1.00e+00 | 4.84e+05 | 0.00e+00 |  1252795 |        0 | 2.38e+04 | 2.75e+04 | 
   -0.73 |          -5.50 |            102 |    46652 |      101 | 2.23e-01 | 9.90e-01 | 4.79e+05 | 0.00e+00 |  1252531 |        0 | 2.35e+04 | 2.72e+04 | 
   -0.23 |          -5.00 |            135 |    43746 |      101 | 1.58e-01 | 7.48e-01 | 1.81e+06 | 0.00e+00 |  4759639 |        0 | 8.90e+04 | 9.76e+04 | 
    0.27 |          -4.50 |            416 |    43094 |      101 | 5.06e-02 | 2.43e-01 | 1.10e+06 | 0.00e+00 |  8575076 |        0 | 5.44e+04 | 5.91e+04 | 
    0.77 |          -4.00 |           4025 |    42091 |      101 | 5.11e-03 | 2.51e-02 | 2.60e+06 | 0.00e+00 | 185389919 |        0 | 1.29e+05 | 1.37e+05 | 
    1.27 |          -3.50 |         101324 |    41813 |      101 | 2.01e-04 | 9.97e-04 | 1.82e+06 | 0.00e+00 | 3878747176 |        0 | 8.86e+04 | 8.67e+04 | 


==> plots/mine/Q7168.tex <==
% |-------|-------------- |-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |  FMEMA   |  BMEMA   |   MBMEM  |   MFMEM  |   FLOPS  |   BOPS   |
% |-------|---------------|-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
   -0.56 |          -6.00 |            109 |    43610 |      101 | 1.95e-01 | 9.27e-01 | 5.89e+05 | 0.00e+00 |  1539562 |        0 | 2.87e+04 | 3.31e+04 | 
   -0.06 |          -5.50 |            246 |    38971 |      101 | 7.74e-02 | 4.11e-01 | 1.80e+06 | 0.00e+00 |  8484766 |        0 | 8.76e+04 | 9.74e+04 | 
    0.44 |          -5.00 |           1601 |    39122 |      101 | 1.19e-02 | 6.31e-02 | 9.99e+05 | 0.00e+00 | 29648191 |        0 | 4.87e+04 | 5.38e+04 | 
    0.94 |          -4.50 |          51451 |    39131 |      101 | 3.71e-04 | 1.96e-03 | 1.82e+06 | 0.00e+00 | 2087722462 |        0 | 8.64e+04 | 8.51e+04 | 


==> plots/mine/Q8192.tex <==
% |-------|-------------- |-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |  FMEMA   |  BMEMA   |   MBMEM  |   MFMEM  |   FLOPS  |   BOPS   |
% |-------|---------------|-----------------|----------|----------|----------|----------|----------|----------|----------|----------|----------|----------|
    0.02 |          -6.00 |            407 |    37937 |      101 | 4.55e-02 | 2.48e-01 | 2.86e+06 | 0.00e+00 | 21562113 |        0 | 1.38e+05 | 1.53e+05 | 
    0.52 |          -5.50 |           4978 |    37530 |      101 | 3.68e-03 | 2.03e-02 | 2.43e+06 | 0.00e+00 | 223972274 |        0 | 1.18e+05 | 1.31e+05 | 
   1.02 |          -5.00 |         118173 |    33951 |       88 | 1.40e-04 | 7.45e-04 | 9.37e+05 | 0.00e+00 | 2508623596 | 

==> plots/theirs/2048.tex <==
% |-------|-------------- |-----------------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |
% |-------|---------------|-----------------|----------|----------|----------|----------|
   -1.50 |          -1.50 |            101 |    51656 |      101 | 2.50e-01 | 1.00e+00 | 
   -1.25 |          -1.25 |            101 |    51752 |      101 | 2.50e-01 | 1.00e+00 | 
   -1.00 |          -1.00 |            101 |    51317 |      101 | 2.48e-01 | 1.00e+00 | 
   -0.75 |          -0.75 |            101 |    51382 |      101 | 2.48e-01 | 1.00e+00 | 
   -0.50 |          -0.50 |            101 |    51155 |      101 | 2.47e-01 | 1.00e+00 | 
   -0.25 |          -0.25 |            101 |    51052 |      101 | 2.47e-01 | 1.00e+00 | 
    0.00 |           0.00 |            101 |    50907 |      101 | 2.46e-01 | 1.00e+00 | 
    0.25 |           0.25 |            102 |    49203 |      101 | 2.36e-01 | 9.90e-01 | 
    0.50 |           0.50 |            114 |    45709 |      101 | 1.96e-01 | 8.86e-01 | 
    0.75 |           0.75 |            133 |    43783 |      101 | 1.61e-01 | 7.59e-01 | 
    1.00 |           1.00 |            269 |    36694 |      101 | 6.66e-02 | 3.75e-01 | 
    1.25 |           1.25 |            642 |    31828 |      101 | 2.42e-02 | 1.57e-01 | 
    1.50 |           1.50 |           2360 |    31542 |      101 | 6.53e-03 | 4.28e-02 | 
    1.75 |           1.75 |          13481 |    30679 |      101 | 1.11e-03 | 7.49e-03 | 
    2.00 |           2.00 |          81682 |    23698 |      101 | 1.42e-04 | 1.24e-03 | 
    2.25 |           2.25 |         911545 |    23437 |      101 | 1.26e-05 | 1.11e-04 | 
    2.50 |           2.50 |        6319204 |    32070 |      101 | 2.48e-06 | 1.60e-05 | 


==> plots/theirs/3072.tex <==
% 3072 
% |-------|-------------- |-----------------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |
% |-------|---------------|-----------------|----------|----------|----------|----------|
   -5.24 |          -7.00 |            101 |    51805 |      101 | 2.50e-01 | 1.00e+00 | 
   -4.99 |          -6.75 |            101 |    51766 |      101 | 2.50e-01 | 1.00e+00 | 
   -4.74 |          -6.50 |            101 |    51902 |      101 | 2.51e-01 | 1.00e+00 | 
   -4.49 |          -6.25 |            101 |    51642 |      101 | 2.50e-01 | 1.00e+00 | 
   -4.24 |          -6.00 |            101 |    51524 |      101 | 2.49e-01 | 1.00e+00 | 
   -3.99 |          -5.75 |            101 |    51684 |      101 | 2.50e-01 | 1.00e+00 | 
   -3.74 |          -5.50 |            101 |    51599 |      101 | 2.49e-01 | 1.00e+00 | 
   -3.49 |          -5.25 |            101 |    51642 |      101 | 2.50e-01 | 1.00e+00 | 
   -3.24 |          -5.00 |            101 |    51398 |      101 | 2.48e-01 | 1.00e+00 | 
   -2.99 |          -4.75 |            101 |    51831 |      101 | 2.51e-01 | 1.00e+00 | 
   -2.74 |          -4.50 |            101 |    51445 |      101 | 2.49e-01 | 1.00e+00 | 
   -2.49 |          -4.25 |            101 |    51802 |      101 | 2.50e-01 | 1.00e+00 | 
   -2.24 |          -4.00 |            101 |    51392 |      101 | 2.48e-01 | 1.00e+00 | 
   -1.99 |          -3.75 |            101 |    51585 |      101 | 2.49e-01 | 1.00e+00 | 
   -1.74 |          -3.50 |            101 |    51582 |      101 | 2.49e-01 | 1.00e+00 | 
   -1.49 |          -3.25 |            101 |    51552 |      101 | 2.49e-01 | 1.00e+00 | 
   -1.24 |          -3.00 |            101 |    51440 |      101 | 2.49e-01 | 1.00e+00 | 
   -0.99 |          -2.75 |            101 |    51035 |      101 | 2.47e-01 | 1.00e+00 | 
   -0.74 |          -2.50 |            101 |    50902 |      101 | 2.46e-01 | 1.00e+00 | 
   -0.49 |          -2.25 |            101 |    49859 |      101 | 2.41e-01 | 1.00e+00 | 
   -0.24 |          -2.00 |            103 |    48171 |      101 | 2.28e-01 | 9.81e-01 | 
    0.01 |          -1.75 |            116 |    44934 |      101 | 1.89e-01 | 8.71e-01 | 
    0.26 |          -1.50 |            167 |    40403 |      101 | 1.18e-01 | 6.05e-01 | 
    0.51 |          -1.25 |            338 |    41028 |      101 | 5.93e-02 | 2.99e-01 | 
    0.76 |          -1.00 |            854 |    37491 |      101 | 2.14e-02 | 1.18e-01 | 
    1.01 |          -0.75 |           3525 |    36045 |      101 | 4.99e-03 | 2.87e-02 | 
    1.26 |          -0.50 |          15653 |    33478 |      101 | 1.04e-03 | 6.45e-03 | 
    1.51 |          -0.25 |         107553 |    37276 |      101 | 1.69e-04 | 9.39e-04 | 
    1.76 |           0.00 |        1203784 |    33351 |      101 | 1.35e-05 | 8.39e-05 | 


==> plots/theirs/384.tex <==
#     Es/N0 |    Eb/N0 ||      FRA |       BE |       FE |      BER |      FER ||  SIM_THR |    ET/RT 
#      (dB) |     (dB) ||          |          |          |          |          ||   (Mb/s) | (hhmmss) 
     -6.00 |    -1.23 ||      112 |     4344 |      112 | 3.03e-01 | 1.00e+00 ||    0.126 | 00h00'00   
      -5.50 |    -0.73 ||      114 |     3867 |      111 | 2.65e-01 | 9.74e-01 ||    0.207 | 00h00'00   
      -5.00 |    -0.23 ||      120 |     3482 |      111 | 2.27e-01 | 9.25e-01 ||    0.241 | 00h00'00   
      -4.50 |     0.27 ||      147 |     2886 |      110 | 1.53e-01 | 7.48e-01 ||    0.369 | 00h00'00   
      -4.00 |     0.77 ||      450 |     6223 |      249 | 1.08e-01 | 5.53e-01 ||    0.607 | 00h00'00   
      -3.50 |     1.27 ||      565 |     3462 |      157 | 4.79e-02 | 2.78e-01 ||    0.511 | 00h00'00   
      -3.00 |     1.77 ||     1159 |     1881 |      102 | 1.27e-02 | 8.80e-02 ||    1.407 | 00h00'00   
      -2.50 |     2.27 ||     5433 |     1811 |      102 | 2.60e-03 | 1.88e-02 ||    2.155 | 00h00'00   
      -2.00 |     2.77 ||    42310 |     1507 |      101 | 2.78e-04 | 2.39e-03 ||    2.560 | 00h00'02   
      -1.50 |     3.27 ||   689775 |     1285 |      100 | 1.46e-05 | 1.45e-04 ||    2.569 | 00h00'34 

==> plots/theirs/4096.tex <==
% 3072 4096 
% |-------|-------------- |-----------------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |
% |-------|---------------|-----------------|----------|----------|----------|----------|
   -3.99 |          -7.00 |            101 |    51583 |      101 | 2.49e-01 | 1.00e+00 | 
   -3.74 |          -6.75 |            101 |    51840 |      101 | 2.51e-01 | 1.00e+00 | 
   -3.49 |          -6.50 |            101 |    51643 |      101 | 2.50e-01 | 1.00e+00 | 
   -3.24 |          -6.25 |            101 |    51726 |      101 | 2.50e-01 | 1.00e+00 | 
   -2.99 |          -6.00 |            101 |    51694 |      101 | 2.50e-01 | 1.00e+00 | 
   -2.74 |          -5.75 |            101 |    51652 |      101 | 2.50e-01 | 1.00e+00 | 
   -2.49 |          -5.50 |            101 |    51349 |      101 | 2.48e-01 | 1.00e+00 | 
   -2.24 |          -5.25 |            101 |    51402 |      101 | 2.49e-01 | 1.00e+00 | 
   -1.99 |          -5.00 |            101 |    51814 |      101 | 2.50e-01 | 1.00e+00 | 
   -1.74 |          -4.75 |            101 |    51683 |      101 | 2.50e-01 | 1.00e+00 | 
   -1.49 |          -4.50 |            101 |    51448 |      101 | 2.49e-01 | 1.00e+00 | 
   -1.24 |          -4.25 |            101 |    51254 |      101 | 2.48e-01 | 1.00e+00 | 
   -0.99 |          -4.00 |            101 |    50461 |      101 | 2.44e-01 | 1.00e+00 | 
   -0.74 |          -3.75 |            101 |    48752 |      101 | 2.36e-01 | 1.00e+00 | 
   -0.49 |          -3.50 |            106 |    46137 |      101 | 2.13e-01 | 9.53e-01 | 
   -0.24 |          -3.25 |            120 |    42213 |      101 | 1.72e-01 | 8.42e-01 | 
    0.01 |          -3.00 |            173 |    39952 |      101 | 1.13e-01 | 5.84e-01 | 
    0.26 |          -2.75 |            456 |    34534 |      101 | 3.70e-02 | 2.21e-01 | 
    0.51 |          -2.50 |           1816 |    32847 |      101 | 8.83e-03 | 5.56e-02 | 
    0.76 |          -2.25 |           7956 |    24857 |      101 | 1.53e-03 | 1.27e-02 | 
    1.01 |          -2.00 |          58919 |    21999 |      101 | 1.82e-04 | 1.71e-03 | 
    1.26 |          -1.75 |         348924 |    16182 |      101 | 2.26e-05 | 2.89e-04 | 
    1.51 |          -1.50 |        4020237 |    15488 |      101 | 1.88e-06 | 2.51e-05 | 

==> plots/theirs/5120.tex <==
% |-------|-------------- |-----------------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |
% |-------|---------------|-----------------|----------|----------|----------|----------|
   -3.02 |          -7.00 |            101 |    51389 |      101 | 2.48e-01 | 1.00e+00 | 
   -2.77 |          -6.75 |            101 |    51755 |      101 | 2.50e-01 | 1.00e+00 | 
   -2.52 |          -6.50 |            101 |    51643 |      101 | 2.50e-01 | 1.00e+00 | 
   -2.27 |          -6.25 |            101 |    51608 |      101 | 2.49e-01 | 1.00e+00 | 
   -2.02 |          -6.00 |            101 |    51614 |      101 | 2.50e-01 | 1.00e+00 | 
   -1.77 |          -5.75 |            101 |    51830 |      101 | 2.51e-01 | 1.00e+00 | 
   -1.52 |          -5.50 |            101 |    51090 |      101 | 2.47e-01 | 1.00e+00 | 
   -1.27 |          -5.25 |            101 |    51016 |      101 | 2.47e-01 | 1.00e+00 | 
   -1.02 |          -5.00 |            101 |    50654 |      101 | 2.45e-01 | 1.00e+00 | 
   -0.77 |          -4.75 |            102 |    49211 |      101 | 2.36e-01 | 9.90e-01 | 
   -0.52 |          -4.50 |            109 |    47512 |      101 | 2.13e-01 | 9.27e-01 | 
   -0.27 |          -4.25 |            127 |    45373 |      101 | 1.74e-01 | 7.95e-01 | 
   -0.02 |          -4.00 |            199 |    42874 |      101 | 1.05e-01 | 5.08e-01 | 
    0.23 |          -3.75 |            435 |    42336 |      101 | 4.75e-02 | 2.32e-01 | 
    0.48 |          -3.50 |           1220 |    42603 |      101 | 1.71e-02 | 8.28e-02 | 
    0.73 |          -3.25 |           4344 |    40143 |      101 | 4.51e-03 | 2.33e-02 | 
    0.98 |          -3.00 |          39468 |    39860 |      101 | 4.93e-04 | 2.56e-03 | 
    1.23 |          -2.75 |         235323 |    40704 |      101 | 8.45e-05 | 4.29e-04 | 
    1.48 |          -2.50 |        2618427 |    38886 |      101 | 7.25e-06 | 3.86e-05 | 
    

==> plots/theirs/6144.tex <==
% |-------|-------------- |-----------------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |
% |-------|---------------|-----------------|----------|----------|----------|----------|
   -2.23 |          -7.00 |            101 |    51316 |      101 | 2.48e-01 | 1.00e+00 | 
   -1.98 |          -6.75 |            101 |    51075 |      101 | 2.47e-01 | 1.00e+00 | 
   -1.73 |          -6.50 |            101 |    51092 |      101 | 2.47e-01 | 1.00e+00 | 
   -1.48 |          -6.25 |            101 |    50163 |      101 | 2.43e-01 | 1.00e+00 | 
   -1.23 |          -6.00 |            101 |    49613 |      101 | 2.40e-01 | 1.00e+00 | 
   -0.98 |          -5.75 |            101 |    48954 |      101 | 2.37e-01 | 1.00e+00 | 
   -0.73 |          -5.50 |            102 |    47738 |      101 | 2.29e-01 | 9.90e-01 | 
   -0.48 |          -5.25 |            111 |    46270 |      101 | 2.04e-01 | 9.10e-01 | 
   -0.23 |          -5.00 |            144 |    44796 |      101 | 1.52e-01 | 7.01e-01 | 
    0.02 |          -4.75 |            228 |    44334 |      101 | 9.49e-02 | 4.43e-01 | 
    0.27 |          -4.50 |            451 |    43846 |      101 | 4.75e-02 | 2.24e-01 | 
    0.52 |          -4.25 |           1362 |    43775 |      101 | 1.57e-02 | 7.42e-02 | 
    0.77 |          -4.00 |           5221 |    44023 |      101 | 4.12e-03 | 1.93e-02 | 
    1.02 |          -3.75 |          24092 |    44800 |      101 | 9.08e-04 | 4.19e-03 | 
    1.27 |          -3.50 |         221477 |    45160 |      101 | 9.96e-05 | 4.56e-04 | 
    1.52 |          -3.25 |        2392580 |    42340 |      101 | 8.64e-06 | 4.22e-05 | 


==> plots/theirs/7168.tex <==
% |-------|-------------- |-----------------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |
% |-------|---------------|-----------------|----------|----------|----------|----------|
   -1.56 |          -7.00 |            101 |    50287 |      101 | 2.43e-01 | 1.00e+00 | 
   -1.31 |          -6.75 |            101 |    49611 |      101 | 2.40e-01 | 1.00e+00 | 
   -1.06 |          -6.50 |            101 |    48764 |      101 | 2.36e-01 | 1.00e+00 | 
   -0.81 |          -6.25 |            104 |    46615 |      101 | 2.19e-01 | 9.71e-01 | 
   -0.56 |          -6.00 |            110 |    43753 |      101 | 1.94e-01 | 9.18e-01 | 
   -0.31 |          -5.75 |            159 |    40521 |      101 | 1.24e-01 | 6.35e-01 | 
   -0.06 |          -5.50 |            260 |    40332 |      101 | 7.57e-02 | 3.88e-01 | 
    0.19 |          -5.25 |            624 |    40237 |      101 | 3.15e-02 | 1.62e-01 | 
    0.44 |          -5.00 |           2362 |    39966 |      101 | 8.26e-03 | 4.28e-02 | 
    0.69 |          -4.75 |          11419 |    37724 |      101 | 1.61e-03 | 8.84e-03 | 
    0.94 |          -4.50 |          79150 |    36881 |      101 | 2.28e-04 | 1.28e-03 | 
   1.19 |          -4.25 |         699712 |    39808 |      101 | 2.78e-05 | 1.44e-04 | 


==> plots/theirs/8192.tex <==
 % |-------|-------------- |-----------------|----------|----------|----------|----------|
  | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      BER |      FER |
% |-------|---------------|-----------------|----------|----------|----------|----------|
   -0.98 |          -7.00 |            101 |    47471 |      101 | 2.29e-01 | 1.00e+00 | 
   -0.73 |          -6.75 |            106 |    44911 |      101 | 2.07e-01 | 9.53e-01 | 
   -0.48 |          -6.50 |            136 |    40379 |      101 | 1.45e-01 | 7.43e-01 | 
   -0.23 |          -6.25 |            189 |    39824 |      101 | 1.03e-01 | 5.34e-01 | 
    0.02 |          -6.00 |            479 |    36444 |      101 | 3.72e-02 | 2.11e-01 | 
    0.27 |          -5.75 |           1354 |    35146 |      101 | 1.27e-02 | 7.46e-02 | 
    0.52 |          -5.50 |           6214 |    36877 |      101 | 2.90e-03 | 1.63e-02 | 
    0.77 |          -5.25 |          52050 |    36300 |      101 | 3.41e-04 | 1.94e-03 | 
    1.02 |          -5.00 |         375312 |    34132 |      101 | 4.44e-05 | 2.69e-04 | 
    1.27 |          -4.75 |        4176888 |    30125 |      101 | 3.52e-06 | 2.42e-05 | 
